On $\ell_p$-hyperparameter Learning via Bilevel Nonsmooth Optimization

We propose a bilevel optimization strategy for selecting the best hyperparameter value for the nonsmooth $\ell_p$ regularizer with $0<p\le 1$. The concerned bilevel optimization problem has a nonsmooth, possibly nonconvex, $\ell_p$-regularized problem as the lower-level problem. Despite the recent popularity of nonconvex $\ell_p$-regularizer and the usefulness of bilevel optimization for selecting hyperparameters, algorithms for such bilevel problems have not been studied because of the difficulty of $\ell_p$-regularizer. Our contribution is the proposal of the first algorithm equipped with a theoretical guarantee for finding the best hyperparameter of $\ell_p$-regularized supervised learning problems. Specifically, we propose a smoothing-type algorithm for the above mentioned bilevel optimization problems and provide a theoretical convergence guarantee for the algorithm. Indeed, since optimality conditions are not known for such bilevel optimization problems so far, new necessary optimality conditions, which are called the SB-KKT conditions, are derived and it is shown that a sequence generated by the proposed algorithm actually accumulates at a point satisfying the SB-KKT conditions under some mild assumptions. The proposed algorithm is simple and scalable as our numerical comparison to Bayesian optimization and grid search indicates.

==> backup/algorithm.tex <==
\section{Smoothing Method for Nonconvex Nonsmooth Bilevel Program}\label{sec:smooth}
For problem \eqref{eqn:bilevel}, one may think of the one-level problem obtained by replacing the lower problem constraint with its first-order optimality condition \citep[10.1~Theorem]{rockafellar2009variational} represented in terms of (general) subgradient%
\footnote{{For precise definitions of a subgradient of a nonconvex function, see Appendix\,\ref{appendix:lemma} in this paper or Chapter~8 of \citep{rockafellar2009variational}.
}}, i.e., 
\begin{equation}
\min_{\w,\blambda}\ f(\w)\hspace{0.5em}\mbox{s.t.}\hspace{0.5em}
\bm 0\in \partial_{\w}(G(\w,\bar{\blambda})+\lambda_1R_1(\w)),\ \blambda \geq \bm 0.\label{eq:0615-2056}
\end{equation}
Notice that $G(\w,\bar{\blambda})+\lambda_1R_1(\w)$ is not convex with respect to $\w$ generally. Hence,
the feasible region of \eqref{eq:0615-2056} can be larger than
that of the original problem \eqref{eqn:bilevel} because not only the global optimal solutions of the lower-level problem but also its local optimal solutions are feasible
solutions for
\eqref{eq:0615-2056}. In that sense, problem \eqref{eq:0615-2056} is modified from the original one, but solving it may lead to better prediction performance because the best hyperparameter $\lambda$ is searched in the wider space
and above all, there is no way to solve the bilevel optimization problem \eqref{eqn:bilevel} as it is.
\subsection{Smoothing method}
In our approach for tackling problem\,\eqref{eqn:bilevel}, we will utilize the smoothing method, which is one of the most powerful methodologies developed for solving nonsmooth equations, nonsmooth optimization problems, and so on. 
Fundamentally, the smoothing method solves smoothed optimization problems 
or equations sequentially to produce a sequence converging to a point that satisfies some optimality conditions of the original nonsmooth problem. 
The smoothed problems solved therein are obtained by replacing the nonsmooth functions with so-called smoothing functions.

Let $\bphi_0:\R^n\to \R$ be a 
nonsmooth function. 
Then, we say that $\bphi:\R^n\times \R_+\to \R$ is a smoothing function of $\bphi_0$ when (i) $\bphi(\cdot,\cdot)$ is continuous and $\bphi(\cdot,\mu)$ is continuously differentiable for any $\mu>0$; 
(ii) $\lim_{\tilde{\w}\to \w,\mu\to 0+}\bphi(\tilde{\w},\mu)=\bphi_0(\w)$ for any $\w\in \R^n$.
In particular, we call $\mu\ge 0$ a smoothing parameter.
{For more details on smoothing methods, see the comprehensive survey article\,\citep{chen2012smoothing} and also relevant articles \citep{nesterov2005smooth,beck2012smoothing}.
%\COMM{AT}{for what?}. 
  \subsection{Our approach}
We propose a smoothing based method for solving \eqref{eqn:bilevel}. 
In the method, we replace the nonsmooth, possibly nonconvex, term  $R_1(\bm w)=\|\bm w\|_p^p$ in \eqref{eqn:bilevel}
by the following smoothing function:
\[
\varphi_\mu(\bm w):=\sum_{i=1}^n (w_i^2+\,\mu^2)^{\frac{p}{2}}.
\]
We then have the following bilevel problem approximating the original one\,\eqref{eqn:bilevel}:
\begin{equation}
\min_{\w^*_{\bm\lambda},\blambda}\ f({\w^*_{\bm\lambda}})\hspace{0.5em}\mbox{s.t.}\hspace{0.5em}\displaystyle {\w^*_{\bm\lambda}} \in \argmin_{\bm w \in \R^n}\left(G(\bm w,\bar{\blambda})+\lambda_1\varphi_{\mu}(\w)\right),\ \bm \lambda \geq \bm 0\notag%\label{eq:smoothed_bilevel}
\end{equation}
which {naturally} leads 
to the following one-level problem:
\begin{align}
\hspace{-2em}\begin{array}{rcc}
\displaystyle \min_{\bm w,\bm \lambda} && f(\bm  w) \\
\mbox{s.t.} && \displaystyle\nabla_{\w} G(\bm w,\bar{\bm \lambda})+ \lambda_1 \nabla \varphi_{\mu}(\bm w)  = \bm 0\\
&& \blambda\ge \bm 0.
\end{array}\label{eqn:smoothprob}
\end{align}
{Note that problem\,\eqref{eqn:smoothprob} is smooth since 
the function $\varphi_{\mu}$ is twice continuously differentiable
\footnote{Huber's function\,\citep{beck2012smoothing} is a popular smoothing function of $R_1(\cdot)$,
but is not twice continuously differentiable.}
when $\mu\neq 0$.
Hence, we can consider the Karush-Kuhn-Tucker (KKT) conditions for this problem.

Let us explain the proposed method in detail.
To this end, for a parameter $\hat{\varepsilon}>0$, we define an $\hat{\varepsilon}$-approximate KKT point 
for problem\,\eqref{eqn:smoothprob}.
We say that 
$(\w,\blambda,\bzeta,\bbeta)\in \R^n\times \R^r\times \R^n\times \R^r$ is 
an $\hat{\varepsilon}$-approximate KKT point
for \eqref{eqn:smoothprob}
if there exists a vector 
$(\bm\varepsilon_1,\varepsilon_2,{\bm \varepsilon}_3,{\bm\varepsilon}_4,\varepsilon_5)\in \R^{n}\times\R\times \R^{r-1}\times \R^n\times \R$ such that
\begin{eqnarray}
&\hspace{-3em}\nabla f(\bm  w) +\left(\nabla_{\w\w}^2 G(\w,\bar{\blambda}) + 
\lambda_1 \nabla^2\bphi_{\mu}(\w)\right){\bm\zeta}=\bm \varepsilon_1,
\label{eq:1215-1}
\\
&\nabla\bphi_{\mu}(\w)^{\top}\bzeta-\eta_1=\varepsilon_2,\label{eqn:1217-1}\\
&\nabla R_i(\w)^{\top}\bzeta-\eta_i=(\bm \varepsilon_3)_i\ \ (i=2,3,\ldots,r),\label{eqn:1217-2}\\
&\nabla_{\w} G(\w,\bar{\blambda})+\lambda_1\nabla\bphi_{\mu}(\w)=\bm \varepsilon_4,\label{eq:1215-2}\\
& \bm 0\le \blambda, ~ \bm 0 \le \bbeta, ~ \blambda^\top \bbeta=\varepsilon_5, \label{eq:1215-3}
\end{eqnarray}
and 
{$$
\|(\bm\varepsilon_1,\varepsilon_2,{\bm \varepsilon}_3,{\bm\varepsilon}_4,\varepsilon_5)\|\le \hat{\varepsilon},$$}
{where $\nabla_{\w\w}^2 G(\w,\bar{\blambda})$ is the Hessian of $G$ with respect to $\w$.}
{\begin{algorithm}[tb]
\caption{Smoothing Method for Nonsmooth Bilevel Program}
\label{alg:smoothing}
\begin{algorithmic}[1]
\REQUIRE
Choose $\mu_0\neq 0$, ${\beta_1,\beta_2} \in (0,1)$ and $\hat{\varepsilon}_0\ge 0$.
Set $k \leftarrow0$.
\REPEAT 
\STATE
{Find an $\hat{\varepsilon}_k$-approximate KKT point {$(\w^{k+1}, \blambda^{k+1},\bzeta^{k+1},\bbeta^{k+1})$} 
for problem\,\eqref{eqn:smoothprob} with $\mu=\mu_k$.}
\STATE
{Update the smoothing and error parameters by $\mu_{k+1} \leftarrow{\beta_1} \mu_k$
and 
$\hat{\varepsilon}_{k+1} \leftarrow {\beta_2} \hat{\varepsilon}_k$.
} 
\STATE $k \leftarrow k+1$.
\UNTIL {convergence of $(\w^k, \blambda^k,\bzeta^{k},\bbeta^{k})$.} 
\end{algorithmic}
\end{algorithm}}
Notice that an $\hat{\varepsilon}$-approximate KKT point is nothing but a KKT point%
\footnote{Note that 
\eqref{eqn:1217-1} and \eqref{eqn:1217-2} with $(\varepsilon_2,({\bm \varepsilon}_3)_2,\ldots,
({\bm \varepsilon}_3)_r)=\bm 0$
can be obtained from 
$$
\nabla_{\blambda}f(\w)+\nabla_{\blambda}
\left(
\left(
\nabla_{\w}
G(\w,\bar{\blambda})+\lambda_1\nabla\varphi_{\mu}(\w)\right)^{\top}\bzeta\right)-\bbeta = \0.
$$
}
for problem\,\eqref{eqn:smoothprob} if $\hat{\varepsilon}=0$.
Hence, }
$\bzeta\in \R^{n}$ and $\bbeta\in \R^r$
are {regarded as approximate} Lagrange multiplier vectors corresponding to 
the equality constraint 
$\nabla_{\w}G(\w,\bar{\blambda})+\lambda_1 \nabla\bphi_{\mu}(\w)=\bm 0$
and the inequality constraints $\blambda\ge \bm 0$, respectively.
{The proposed algorithm produces a sequence of $\hat{\varepsilon}$-approximate KKT points 
for problem\,\eqref{eqn:smoothprob} while decreasing the values of $\hat{\varepsilon}$ and $\mu$ to $0$.
Precisely, it is described as in Algorithm\,\ref{alg:smoothing}.}

Though, in Algorithm\,\ref{alg:smoothing}, we do not designate any means for computing an $\hat{\varepsilon}$-approximate KKT point for \eqref{eqn:smoothprob},
  sequential quadratic programming (SQP) methods\,\citep{nocedal2006numerical} are promising candidates.
  However, since such SQP methods are designed for solving general constrained problems, we may develop more efficient algorithms by exploiting structure of individual problems.
  This issue will be discussed later in Section~\ref{sec:numeric}.
    See also Appendix\,\ref{appendix:B}.
As for practical stopping criteria of Algorithm~1, we make use of the scaled bilevel SB-KKT conditions studied in the subsequent section.



==> backup/numericalexp.tex <==
\section{Numerical Experiments}\label{sec:numeric}
In this section, we investigate the performance of Algorithm~\ref{alg:smoothing} through comparison to other hyperparameter learning methods such as Bayesian optimization\,\citep{Mockus1978} and gridsearch.
All the experiments are conducted on a personal computer with
  Intel Core i7-8559U CPU @ 2.70GHz, 16.00 GB memory.  
Algorithm~\ref{alg:smoothing} and the other competitor algorithms are implemented with MATLAB R2020a.

Two kinds of bilevel problems relevant to linear regression with real data are solved.
The first problem handles a single hyperparameter related to the $\ell_p$-regularizer, while the second one does multiple hyperparameters.
\subsection{Linear regression bilevel problem with a single $\ell_p$ hyperparameter}\label{sec:single}
In this section, we solve the following bilevel problem regarding squared linear regression problem with a single $\ell_p$ hyperparameter.
\begin{align}\label{al:0913}
\begin{array}{rll}
\displaystyle{\min_{\bw,\blambda}}&\ &\|\bA_{\rm val}{\w}-\bm b_{\rm val}\|_2^2\\ 
\mbox{s.t. }&  &\bw \in \displaystyle{\mathop{\rm argmin}_{\hat{\bw}}}\ \left(\|\bA_{\rm tr}\hat{\w}-\bm b_{\rm tr}\|_2^2 + {\exp(\lambda_1)\|\hat{\bw}\|_p^p}
\right),\\
\end{array}
\end{align}
where $p\in (0,1]$ and $(\bA_{\rm txt},\bm b_{\rm txt})\in \R^{m_{\rm txt}\times n}\times \R^{m_{\rm txt}}$ for ${\rm txt}\in \{{\rm val,tr}\}$.
Notice that the form of the above problem slightly differs from that of \eqref{eqn:bilevel} in that $\lambda_i$ is replaced with $\exp(\lambda_i)$ for each~$i$.
  This is because positive hyperparameters, in particular $\lambda_1$, are actually desirable as outputs.
  With this manipulation, the nonnegative constraint $\exp(\lambda_i)\ge \0$, which corresponds to $\lambda_i\ge \0$ in \eqref{eqn:bilevel}, is clearly fulfilled and thus removed.

   For the sake of examining the accuracy of solutions obtained by solving the above problem, we use
  $\|\bA_{\rm te}\w-\bm b_{\rm te}\|_2^2$ as a test error function, where $\bA_{\rm te}\in \R^{m_{\rm te}\times n}$ and $\bm b_{\rm te}\in \R^{m_{\rm te}}$.
The data matrices and vectors $\bA_{\{{\rm val,tr,te}\}}, \bm b_{\{{\rm val,tr,te}\}}$ are taken from UCI machine learning repository\,\cite{Lichman:2013}:
{\bf Facebook} Comment Volume ($\bar{m}=40949$, $n=53$), 
{\bf Insurance} Company Benchmark ($\bar{m}=9000$, $n= 85$),
%{\bf Online} News Popularity ($\bar{m}=39797$, $\bar{n}= 61$),
{\bf Student} Performance for a math exam ($\bar{m}={395}$, $n= 272$)\footnote{The original dataset has $n= 32$, but the feature size is increased by adding new features: interaction effects generated by pairwise products among some features for each sample.},
%{\bf Communities} and Crime ($\bar{m}=1994$, $n= 1955$)\footnote{Originally, $n= 127$, but the feature size was increased by expressing the qualitative variables with dummy variables.},
{{\bf BodyFat} ($\bar{m}=336$, $n= 14$), 
and
{\bf CpuSmall} ($\bar{m}=8192$, $n= 12$)} are from UCI machine learning repository \cite{Lichman:2013}.
The $\bar{m}$ samples are divided into 3 groups
(training, validation and test samples) with the same sample size {$\lceil\bar{m}/3 \rceil$}.
Hence, $m_{\{{\rm val,tr,te}\}}=\lceil\bar{m}/3 \rceil$.

\subsubsection{Experimental conditions}
{\paragraph{Method for solving the smoothed subproblem\,\eqref{eqn:smoothprob}:}
Algorithm~\ref{alg:smoothing} requires an $\hat{\varepsilon}$-approximate KKT point of \eqref{eqn:smoothprob} in Step~2 at every iteration.
To compute such a point, we present an algorithm using implicit functions.
Several past works also employed similar approaches based on implicit functions for hyperparameter optimization. For example, see \citep{maclaurin2015gradient,pmlr-v48-pedregosa16,franceschi2018bilevel}.

We only explain the algorithmic framework of the proposed implicit function based method, leaving the precise description to Algorithm~\ref{alg_subproblem0} in Appendix~\ref{appendix:B1}.
At every iteration, Algorithm~\ref{alg_subproblem0} locally represents problem\,\eqref{eqn:smoothprob} as problem having the hyperparameter $\blambda$ as variables by means of implicit functions defined over the $\blambda$-space.  
The implicit function, say $\w(\cdot)$, is defined on some open set $U$ and expresses a solution set for the smoothed lower-level problem 
$\min_{\bm w \in \R^n} G(\bm w,\bar{\blambda})+\lambda_1\varphi_{\mu}(\w)$. Namely,
we have $\displaystyle\nabla_{\w} G(\bm w(\blambda),\bar{\bm \lambda})+ \lambda_1 \nabla \varphi_{\mu}(\bm w(\blambda))  = \bm 0$ for all $\blambda\in U$.
We then solve the reformulated problem\,\eqref{eqn:smoothprob} that is described in terms of $\blambda$ by the quasi-Newton method\,\citep{nocedal2006numerical}.
Note that, though it is difficult in general to know the concrete form of the implicit function $\w(\cdot)$,
we can compute the gradient $\nabla\w$ in virtue of the implicit function theorem, which enables us to perform gradient based methods like the quasi-Newton method for solving problems that are described in terms of $\w(\cdot)$. 


Actually, the efficiency of this approach relies on how rapidly and accurately $\w(\blambda)$ is computed for a given $\blambda$. To this end, we employ a certain modified Newton method, which was originally proposed by \citet{lai2011unconstrained}. See Appendix~\ref{appendix:B2} for details.

Moreover, as a starting point of the algorithm,
we use a solution of the smoothed problem\,\eqref{eqn:smoothprob} at the previous iteration of Algorithm~\ref{alg:smoothing}, aiming for the so-called hot-start effect.}
\paragraph{Other algorithms for comparison:}
For the sake of comparison, we also implement Bayesian optimization and the gridsearch method. 
We use \texttt{bayesopt} in MATLAB with ``MaxObjectiveEvaluations=30'' for Bayesian optimization.
{In gridsearch, we search for the best value of $\|\bA_{\rm val}{\w}-\bm b_{\rm val}\|_2^2$ among 30 grids $\lambda =10^{-4},10^{-4+\frac{8}{29}},\cdots,10^{4-\frac{8}{29}},10^{4}$ for problem\,\eqref{al:0913}.
At each iteration of \texttt{bayesopt} and gridsearch, we
make use of Matlab built-in solver~\texttt{fmincon} so as to solve the lower-level problem of \eqref{al:0913} with a given $\bm \lambda$. 

\paragraph{Parameter setting and termination criteria:}
The smoothing parameter in Algorithm~\ref{alg:smoothing}
is initialized as $\mu_0=1$ and updated by $\mu_{k+1}=\min(0.9\mu_k,10\mu_k^{1.3})$.
The smoothed subproblem~\eqref{eqn:smoothprob} is solved as exactly as possible by fixing $(\hat{\varepsilon}_{0},\beta_0)$ to $(10^{-6},1)$.
As for the termination criteria of Algorithm~\ref{alg:smoothing}, writing a resulting solution as $\w^{\ast}$,
we stop it if the SB-KKT conditions \eqref{eqa:1214-1},
\eqref{eqa:1214-2} and \eqref{eqa:1214-3}
are within the error of $\epsilon:=10^{-3}$.
We also check whether the other SB-KKT conditions\,\eqref{eqa:1214-6}-\eqref{eqa:1214-5} are satisfied.
The default setting of \texttt{bayesopt} is employed. 
Time limits of all the algorithms are set to 600 seconds. }

\subsubsection{Numerical results for problem~\eqref{al:0913} with fixed data size}
{We first show the results of applying the three algorithms to problem~\eqref{al:0913} with $p=1,0.8,0.5$. 
The algorithms are run for 5 times from different starting points $(\blambda^0,\w^0)$ generated in the manner that $\blambda^0$ is set to $\0$ and $\w^0$ is chosen randomly from $[-5,5]^n$.
All the results are summarized in Table~\ref{tbl:comparison_full}, where the value $\mbox{Err}_{\rm te}$ indicates the averaged values of
$\|\bA_{\rm te}\w-\bm b_{\rm te}\|^2$ over 5 runs. The value $\mbox{Err}_{\rm val}$ stands for the averaged value of $\|\bA_{\rm val}\w-\bm b_{\rm val}\|^2$.
The value ``sparsity'' means the ratio of zero elements in the obtained solution $\bm w \in \R^n$, i.e., ${\rm sparsity}=\left|\{i\mid w_i=0\}\right|/n$ and hence, the solution with sparsity$\approx 1$  is very sparse.
We denote by {\rm time(sec)} the spent time from the start to the termination.
In the experiments, for each $i$, we regarded $w_i$ as zero if $|w_i|\le 10^{-4}\max_{1\le i\le n}|w_i|$.
The best (smallest) values of $\mbox{Err}_{\{\rm te,val\}}$ and time(sec), among the three algorithms are displayed in bold.


From the table,  
there are significant differences in time(sec) of the three algorithms, while ${\rm Err}_{\rm te}$ and ${\rm Err}_{\rm val}$ seem comparative. In particular, Algorithm~\ref{alg:smoothing} tends to be the fastest.
Indeed, it attains the best values in time(sec) for 10 out of 15 problem-instances, seven of which moreover achieve the best values in ${\rm Err}_{\rm val}$.
For example, for {\bf Facebook} with $p=1$, it computes a solution with ${\rm Err_{\rm val}}=6.474$ by about 17 seconds, while \texttt{bayesopt} and gridsearch do solutions with ${\rm Err_{\rm val}}\ge 6.476$ after spending more than 40 seconds.
Thus, Algorithm~\ref{alg:smoothing} is likely to be the most effective among the three on seeking $(\w,\blambda)$ with good ${\rm Err}_{\rm val}$.
{\redcolor
  As pointed out by a reviewer, \texttt{bayesopt} actually found the final solutions or close solutions earlier than the recorded time on the table.
%     
  %So, we also investigated how the best observed objective value of \texttt{bayesopt} varies over time.
Nonetheless, in many instances, Algorithm~\ref{alg:smoothing} reached the final solution more quickly than \texttt{bayesopt} found such a solution. 
%But, depending on a problem, we also observed that \texttt{bayesopt} was faster than ours. 
%  but in many cases.    
  %onetheless, we also confirmed that our algorithm is faster to reach the final solution than \texttt{bayesopt} does such 
  %n many cases.
  We refer readers to 
 Table\,\ref{tbl1:appendix} 
 in Appendix~\ref{sec:appC}, which shows the first time of \texttt{bayesopt} for finding a solution which attains the final best observed objective value, i.e., validation value. Also see Figure\,\ref{Fig;0618-1} that depicts the time-series of the best observed objective value of \texttt{bayesopt} for the problem organized with the data sets of {\bf Student} and {\bf CpuSmall}.}


From the values of sparsity, the problems with smaller $p$ tends to output sparser solutions. For example, 
Algorithm~\ref{alg:smoothing} outputs a solution with ${\rm sparsity}\ge 0.9$ for {\bf Facebook} with $p=0.5$, while ${\rm sparsity}\le 0.3$ for $p=0.8,1$. 
Nevertheless, sparsity of Algorithm~\ref{alg:smoothing} is 0.00
for {\bf BodyFat} with $p=0.8$, while 
${\rm sparsity}=0.7, 0.07$ for $p=0.5,1$, respectively. 
In this case, Algorithm~\ref{alg:smoothing} might fall into a local optimum with small $E_{\rm val}$ at the expense of sparsity.}





\subsubsection{Performance with Varied Data Size}
{Changing the data sizes of {\bf Student} and {\bf Facebook} datasets, we make comparison of the performances of Algorithm~\ref{alg:smoothing}, \texttt{bayesopt}, and gridsearch.

  We first examine how ${\rm Err}_{\rm te}$, ${\rm Err}_{\rm val}$, and time(sec) of the three algorithms change against the sample size, $\hat{m}$, of {\bf Facebook}.
  The sample size $\hat{m}$ is increased from $\frac{1}{2}\bar{m}$ to $\bar{m}$ by $\frac{1}{10}\bar{m}$ with $\bar{m}\approx 40000$.
  We apply the algorithms using $\ell_{0.8}$ regularizer to these problems with a varied sample size. The obtained results are depicted in Figure~\ref{fig:lasst}.
  Figures~\ref{fig:last1} and \ref{fig:last2} indicates that the computed test and validation values ${\rm Err}_{\rm te}$ and ${\rm Err}_{\rm val}$ behave analogously as $\hat{m}$ increases. There are no crucial differences among those values. However, from Figure~\ref{fig:last3},
  computation time, time(sec), of \texttt{bayesopt} grows more rapidly than the others. This may be because 
  \texttt{bayesopt} has to search a wider region as the sample size grows.
  In contrast, the values of time(sec) of Algorithm~\ref{alg:smoothing} and gridsearch grow moderately. In particular, Algorithm~\ref{alg:smoothing} is the fastest for most cases.


  
 \begin{figure}[htbp]
 %\pgfimage[width = \hsize]{blog_data_value.eps}
 \begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.5]{test_sample.eps}
 \subcaption{${\rm Err}_{\rm te}$ vs scaled sample size $\hat{m}/\bar{m}$
 }
 \label{fig:last1}
 \end{minipage}%\hfill
 \begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.5]{val_sample.eps}
 \subcaption{${\rm Err}_{\rm val}$ vs scaled sample size $\hat{m}/\bar{m}$
 }
 \label{fig:last2}
 \end{minipage}  \vspace{1em}\\
 \centering
\begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.5]{cputime_sample.eps}
 \subcaption{time(sec) vs scaled sample size $\hat{m}/\bar{m}$
 }
 \label{fig:last3}
 \end{minipage}
 
   \caption{Performance of Algorithm~\ref{alg:smoothing}, \texttt{bayesopt}, and gridsearch using $\ell_{0.8}$ regularizer for
       {\bf Facebook} with fixed feature size $n=53$ and varying sample size $\hat{m}$
       ($\bar{m}=40949$); Alg.1: Algorithm~\ref{alg:smoothing}, bayes: \texttt{bayesopt}, grid: gridsearch},  
 \label{fig:lasst}
 \end{figure}

   Next, we investigate the performances of the algorithms by varying the feature size, $\hat{n}$, of {\bf Student}. As in the above experiment, we use $\ell_{0.8}$ regularizer.
   The feature size $\hat{n}$ is increased from $\frac{1}{2}n$ to $n$ by $\frac{1}{10}n$ with $n=272$.
   The obtained results are shown in Figure~\ref{fig:lasst-2}.
   Algorithm~\ref{alg:smoothing} successfully attains better values in all time(sec), $\mbox{Err}_{\rm te}$, and $\mbox{Err}_{\rm val}$ than \texttt{bayesopt} and gridsearch
   for $n\ge 0.7\hat{n}$. From Figures~\ref{fig:last1-2} and \ref{fig:last2-2}, \texttt{bayesopt} seems stuck in a local optimum with larger
$\mbox{Err}_{\rm val}$ and $\mbox{Err}_{\rm te}$ for $n\ge 0.8\hat{n}$.
   From Figure~\ref{fig:last3-2}, time(sec) for \texttt{bayesopt} and gridsearch grow more rapidly than ours as $\hat{n}$ increases.



The above two experiments suggest that, compared with gridsearch and Bayesian optimization, Algorithm~\ref{alg:smoothing} is unlikely to be affected by growth of the data size. 



 \begin{figure}[htbp]
 %\pgfimage[width = \hsize]{blog_data_value.eps}
 \begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.5]{test_feature.eps}
 \subcaption{${\rm Err}_{\rm te}$ vs scaled feature size $\hat{n}/n$
 %with fixed $n=53$ for {\bf Facebook}
 }
 \label{fig:last1-2}
 \end{minipage}%\hfill
 \begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.5]{val_feature.eps}
 \subcaption{${\rm Err}_{\rm val}$ vs scaled feature size $\hat{n}/n$
 %with fixed $n=53$ for {\bf Facebook}
 }
 \label{fig:last2-2}
 \end{minipage}  \vspace{1em}\\
 \centering
\begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.5]{cpu_feature.eps}
 \subcaption{time(sec) vs scaled feature size $\hat{n}/n$
 %with fixed $n=53$ for {\bf Facebook}
 }
 \label{fig:last3-2}
 \end{minipage}
 
   \caption{Performance of Algorithm~\ref{alg:smoothing}, \texttt{bayesopt}, and gridsearch using $\ell_{0.8}$ regularizer for
{\bf Student} with varying feature size $\hat{n}$ ($n=272$) and fixed sample size $\bar{m}=395$; Alg.1: Algorithm~\ref{alg:smoothing}, bayes: \texttt{bayesopt}, grid: gridsearch} 
 \label{fig:lasst-2}
 \end{figure}   
}









 
  \input{tablewatanabe}
  \subsubsection{Performance as the smoothing parameter $\mu$ decreases}\label{experiment:mu}
{We examine impact of the smoothing parameter $\mu$ on test error of solutions of the smoothed subproblems\,\eqref{eqn:smoothprob}. 
Figures~\ref{fig:last3-3}-\ref{fig:last5-3} depict the growth behavior of the test error in the final stage of Algorithm~\ref{alg:smoothing} for the problems of {\bf Facebook}, {\bf BodyFat}, and {\bf Insurance}.

From the figures, the test errors for the three problems do not vary significantly.
Taking into account that the smoothed subproblem\,\eqref{eqn:smoothprob} is more difficult as $\mu$ becomes smaller,
it may be good strategy to stop the algorithm earlier than convergence to a SB-KKT point.	
This is also indicated by the fact that, around $\mu=0.01$, the algorithm attains solutions with better test errors than the solutions upon termination for {\bf Facebook} and {\bf BodyFat}.}


\begin{figure}[htbp]
 %\pgfimage[width = \hsize]{blog_data_value.eps}
 \begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.48]{face_test_mu.eps}
 \subcaption{{\bf Facebook}
 }
 \label{fig:last3-3}
 \end{minipage}%\hspace{0em}
 \begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.48]{body_test_mu.eps}
 \subcaption{{\bf BodyFat}
 %with fixed $n=53$ for {\bf Facebook}
 }
 \label{fig:last4-3}
 \end{minipage}%\hfill
 \vspace{0.5em}\\
 \centering
  \begin{minipage}{.5\hsize}
 \centering
 \includegraphics[scale = 0.48]{insur_test_mu.eps}
 \subcaption{{\bf Insurance}}
 \label{fig:last5-3}
  \end{minipage}
     \caption{Change of test error for $\ell_{0.8}$ regularizer as 
  $\mu$ decreases; The horizontal axis: a smoothing parameter $\mu$; The vertical axes: test error}
 \label{fig:lasst-3}
 \end{figure} 

{\subsection{Linear regression problem with multiple hyperparameters}
Next, we solve the following problem that possesses multiple hyperparameters:
\begin{align}\label{al:0913-2}
\begin{array}{rll}
\displaystyle{\min_{\bw,\blambda}}&\ &\|\bA_{\rm val}{\w}-\bm b_{\rm val}\|_2^2 \\ 
\mbox{s.t. }&  &\bw \in\displaystyle{\mathop{\rm argmin}_{\hat{\bw}}}\ \left(\|\bA_{\rm tr}\hat{\w}-\bm b_{\rm tr}\|_2^2 + {\exp(\lambda_1)\|\hat{\bw}\|_p^p}
+\hwCw
\right),
\end{array}
\end{align}
where
$\C(\bm \bar{\blambda}):={\rm Diag}(\exp(\lambda_i))_{i=2}^{n+1}$ being positive definite and $\bA_{\{\rm val,tr,te\}}$ and $\bm b_{\{\rm val,tr,te\}}$ are the ones used in the previous experiments in Section~\ref{sec:single}.
\subsubsection{Experimental conditions}
\tred{We set $p=0.5$ in problem\,\eqref{al:0913-2}}.
The experimental conditions are almost the same as those for problem~\eqref{al:0913}. The main differences are as follows:
We make comparison of Bayesian Optimization~\texttt{bayesopt}
\tred{with ``MaxObjectiveEvaluations=300''} and Algorithms~\ref{alg:smoothing} using the two algorithms for solving subproblems~\eqref{eqn:smoothprob}: The first one is the implicit function approach as in the previous experiments and the second one is \texttt{fmincon}, where we opt for the SQP method and set ``MaxIterations$=10^7$''.
Though we also implemented gridsearch seeking a solution over $30^n$ grids $\blambda\in \{10^{-4},10^{-4+\frac{8}{29}},\cdots,10^{4-\frac{8}{29}},10^{4}\}^n$,
the obtained results were actually quite poor because the number of grids, which was larger than $30^{10}$, was too huge to search. We thus omit those results with gridsearch.
Finally, according to the observation in the last experiment in Subsection\,\ref{experiment:mu}, we terminate Algorithm~\ref{alg:smoothing} when $\mu_k\le 0.01$.

\subsubsection{Numerical results for problem~\eqref{al:0913-2}}
Table~\ref{tbl2:comparison_full} summarizes the obtained results of applying the two types of Algorithms~\ref{alg:smoothing} and \texttt{bayesopt} to problem\,\eqref{al:0913-2}.
%the implicit function approach as in the previous experiments for problem\,\eqref{al:0913} and \texttt{fmincon} for solving subproblems~\eqref{eqn:smoothprob}. 
In the table, we denote by $\sharp \blambda$ the number of hyperparameters $\blambda$ in each problem.
Moreover, {\algone} stands for Algorithm~\ref{alg:smoothing} using the implicit function approach and {\algtwo} does the one using \texttt{fmincon}.
The hyphens ``--'' in the line of {\bf Facebook} for {\algtwo} 
indicate that \texttt{fmincon}, which is used in {\algtwo}, terminates with an infeasible solution of the smoothed problem\,\eqref{eqn:smoothprob}.



From the table, compared with the results for the single-hyperparameter bilevel problem\,\eqref{al:0913}, \texttt{bayesopt} does not work well. 
For four out of the five problems, it cannot terminate within the time-limit 600 seconds. The qualities of the output solutions of \texttt{bayesopt} upon termination are
also not good in values of ${\rm Err}_{\rm val}$
and ${\rm Err}_{\rm te}$.
\tred{For the sake of completeness, as well as the previous experiment, we examined
the first time when the best observed objective values, i.e., validation values of \texttt{bayesopt} were found.
%  Although it found a solution as good as the final solution more quickly than the recoded time on the table,
% For example, as to {\bf CpuSmall}, \texttt{bayesopt} reached solutions attaining the validation value $1.8\times 10^5$ around 150 seconds, which is much earlier than the time limit. 
Refer to Table\,\ref{tbl2:appendix} in Appendix\,\ref{sec:appC}.
Also see Figure\,\ref{Fig;0618-2} for graphs depicting the time-series of the best observed objective values concerning the data sets of {\bf Student} and {\bf CpuSmall}.
  %The results of the other data sets showed quite similar tendencies to {\bf Student}.
}

\tred{In contrast to \texttt{bayesopt},} the two Algorithms~\ref{alg:smoothing} with different subroutines show better performance.
There are notable differences between performances of {\algone} and {\algtwo}.
While {\algone} seems to fall into non-sparse solutions, but with good ${\rm Err}_{\{\rm te,val\}}$ for {\bf Insurance}, {\bf BodyFat}, and {\bf CpuSmall}, {\algtwo} finds good solutions balancing in sparsity, ${\rm Err}_{\rm te}$, and ${\rm Err}_{\rm val}$ for all the same data sets.
This may be because {\algone} computes a solution of problem\,\eqref{eqn:smoothprob} by remaining in the feasible set, namely, the solution set of the smoothed lower level problem.
This behavior may cause {\algone} to miss a chance of broadly seeking sparse solutions.} Meanwhile, {\algtwo} using the SQP method in \texttt{fmincon} tends to approach a solution of \eqref{eqn:smoothprob} from the outside of the feasible set,
which often leads to a good solution even in sparsity.
\input{tablewatanabe2}
 


==> backup/tableApp1.tex <==
  \begin{table}[H]
  %\begin{sidewaystable*}[h]
\centering
\caption{%\COMM{AT}{Delete later}
\redcolor The first time of \texttt{bayesopt} for finding a solution of problem\,\eqref{al:0913}, which attains the final best observed objective value, i.e., validation value
(Those results of \texttt{bayesopt} were recorded in a single run, thus differ from the averaged results over 5 runs shown in Table\,\ref{tbl:comparison_full}.
For the sake of comparison, the results of Algorithm~\ref{alg:smoothing} are also shown, which are the same as those in Table\,\ref{tbl:comparison_full}.
``{\ftime}'' stands for the first time in seconds where 
the best objective value is observed.  
The best values in {\ftime} and $\mbox{Err}_{\rm val}$ are displayed in bold.)
}
\label{tbl1:appendix}
	{
\scalebox{1}{%ワタナベが付け加えた
\begin{tabular}{crrrrr}
\toprule
\multicolumn{2}{c}{Data}&
\multicolumn{2}{c}{\texttt{bayesopt}}&
\multicolumn{2}{c}{{\Alg}}\\
\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\multicolumn{1}{c}{name}&
\multicolumn{1}{c}{$p$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{\ftime}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)}\\
\midrule
{\bf Facebook} &1 	&	 6.476& 42.256&  {\bf 6.474}&  {\bf 17.399} \\		
%($\bar{m}=40949$)
	       &　0.8 	&{\bf 6.504}&122.158&  6.512&  {\bf 22.242}\\
%($n=53$)
	　　　&  0.5 	&{\bf 6.536}	& 66.589&6.550   & {\bf 16.820}     \\ \hline
{\bf Insurance} &  1	&	{\bf 95.764}&49.538  	&       {\bf 95.764}  &	{\bf 33.077}  \\
	        & 0.8	&   95.737&   63.580    &	   {\bf 95.676} 	&	{\bf 32.465} 	\\
	        & 0.5 	&95.604		&{\bf 13.960}    &   {\bf 95.562} 	&	44.904  \\ \hline

{\bf Student} 	&  1    &   {\bf 0.777} &12.405      &   0.778 &	{\bf 10.586}    \\
	        & 0.8 	&{\bf 0.724}	&339.980	&  {\bf 0.724} &	{\bf 2.348} 	  \\

　　　　　　　　& 0.5	&0.731	        &147.118	&    {\bf 0.724} &	 {\bf 3.618}\\ \hline
%
{\bf BodyFat} 	&   1	&{\bf 0.209}   & 4.839	& {\bf 0.209} 	&	{\bf 0.068} \\
                & 　0.8	&　 0.180 &3.899	& {\bf 0.179} 	&	{\bf 0.203} \\
& 　0.5 &　　{\bf 0.212}	&1.160 & 0.267 &{\bf 0.395} \\ \hline
%
{\bf CpuSmall} &1 	&    131124&	{\bf 1.202}&  {\bf 130981} 	&	11.299 \\
& 0.8 	&    131187&1.853	& {\bf 130982}&	{\bf 0.741} 	\\
	　　　　& 0.5	&　　131234&1.712	& {\bf 131058} 	&	{\bf 0.672} 	\\ 
\bottomrule
\end{tabular}}}
\end{table}


==> backup/tableApp2.tex <==
\begin{table}[H]
\centering
\caption{
\redcolor The first time of \texttt{bayesopt} for finding a solution of problem\,\eqref{al:0913-2}, which attains the final best observed objective value, i.e., validation value
(Those results of \texttt{bayesopt} were recorded in a single run, thus differ from the averaged results over 5 runs shown in Table\,\ref{tbl2:comparison_full}.
For the sake of comparison, the results of Algorithm~\ref{alg:smoothing} ({\algone}, {\algtwo}) are also shown, which are the same as those in Table\,\ref{tbl2:comparison_full}.
``{\ftime}'' stands for the first time in seconds where 
the best objective value is observed.  
The best values in {\ftime} and $\mbox{Err}_{\rm val}$ are displayed in bold.)
}
\label{tbl2:appendix}
	{
\scalebox{1}{%ワタナベが付け加えた
\begin{tabular}{crrrrrrr}
\toprule
\multicolumn{2}{c}{Data}&
\multicolumn{2}{c}{\texttt{bayesopt}}&
\multicolumn{2}{c}{{\algone}}&
\multicolumn{2}{c}{{\algtwo}}\\
\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\multicolumn{1}{c}{name}&
\multicolumn{1}{c}{$\sharp\blambda$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{\ftime}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)} &
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)}\\
\midrule
{\bf Facebook}				&	54
&	8.780 	&	{\bf 1.518}  
&	{\bf 6.478} 	&	20.247	 	
&	--&	--
\\\hline
{\bf Insurance}					& 86
&	107.000 	&	{\bf 4.288}
&	95.694 	&	{50.714}  	
&	{\bf 94.604} 	&	{4.473}
\\\hline
{\bf Student}				& 273	
&	18.324 	&	26.756 
&	{\bf 0.771} 	&	{\bf 1.451} 
&	0.786 	&	71.775 	\\\hline
{\bf BodyFat}
& 15  
&	46.815 	&	0.337
&	0.243 	&	{\bf 0.072} 	
&	{\bf 0.130} 	&	0.695 \\\hline
{\bf CpuSmall}					
& 13
&	151394 	&	531.837  
&	131130 	&	6.222 
&	{\bf 128540} 	&	{\bf 0.658} \\
\bottomrule
\end{tabular}}}
\end{table}


==> backup/tablewatanabe.tex <==

\begin{landscape}
  \begin{table}[h]
  %\begin{sidewaystable*}[h]
\centering
\caption{%\COMM{AT}{Delete later}
  Comparison of Algorithm~\ref{alg:smoothing}, \texttt{bayesopt} in MATLAB and gridsearch in terms of squared errors (validation error ${\rm Err}_{\rm val}$ and test error ${\rm Err}_{\rm te}$), CPU times (time(sec)), and sparsities (sparsity).
Here, ${\rm sparsity}:=\left|\{i\mid w_i=0\}\right|/n$ and hence 
a solution is sparser as ``{\rm sparsity}'' is closer to 1. 
The best values in ${\rm Err}_{\rm val}$, ${\rm Err}_{\rm te}$, and time(sec) are displayed in bold.}
\label{tbl:comparison_full}
	{
\scalebox{1}{%ワタナベが付け加えた
\begin{tabular}{lrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{2}{c}{Data}&
\multicolumn{4}{c}{{\Alg}}&
%\multicolumn{4}{c}{\texttt{fmincon} based bilevel alg.}&
\multicolumn{4}{c}{\texttt{bayesopt} in MATLAB}&
\multicolumn{4}{c}{grid search}\\
\cmidrule(lr){1-2}
\cmidrule(lr){3-6}
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
\cmidrule(lr){15-18}
\multicolumn{1}{c}{name}&
\multicolumn{1}{c}{$p$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm te}$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)}&
%\multicolumn{1}{c}{\#{} nonzero}&
\multicolumn{1}{c}{sparsity}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm te}$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)} &
\multicolumn{1}{c}{sparsity}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm te}$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)}&
%\multicolumn{1}{c}{\#{} nonzero}&
\multicolumn{1}{c}{sparsity}\\
%\multicolumn{1}{c}{$\mbox{Err}_{te}$}&
%\multicolumn{1}{c}{$\mbox{Err}_{val}$}&
%\multicolumn{1}{c}{time (sec)}&
%%\multicolumn{1}{c}{\#{} nonzero}&
%\multicolumn{1}{c}{sparsity}\\
\midrule
{\bf Facebook} &1 	&	5.399 	&	{\bf 6.474} 	&	{\bf 17.399} 	&	0.057 	
%&5.399 	&	6.475 	&	{\bf 12.441} 	&	0.075 	
&	5.401 	&	6.476 	&	146.144 	&	0.249 	&	{\bf 5.394} 	&	6.483 	&	43.738 	&	0.264 \\		
%($\bar{m}=40949$)
					& 		0.8 	&	5.431 	&	6.512 	&	{\bf 22.242} 	&	0.245 	
					%&	5.484 	&	6.556 	&	{\bf 18.192}	&	0.642 	
					&	{\bf 5.411} 	&	{\bf 6.499} 	&	137.764 	&	0.143 	
					&	5.439 	&	6.545 	&	37.021 	&	0.113 \\
%($n=53$)
					& 		0.5 	&	5.455 	&	6.550 	&	16.820	&	0.925
					 	%&	5.527 	&	6.605 	&	19.300 	&	0.887 	
					 	&	{\bf 5.452}	&	{\bf 6.535} 	&	93.967 	&	0.596
					 	&	5.704 	&	6.747 	&	{\bf 16.514} 	&	0.925 \\ \hline
%					&	\tred{wCw}	&	{\bf 5.404} 	&	6.478 	&	{\bf 20.247}	&	0.038 	
%					        % &	{\bf 5.389}	&	6.464 	&	158.128 	&	0.189 
%	&	(F)7.629 	&	8.780 	&	300.000 	&	0.000 	&	---	&	---	&	---	&---	\\\hline  
{\bf Insurance}      			& 		1	&	 {\bf 87.837} 	&	{\bf 95.764} 	&	33.077 	&	0.035 	
%&	{\bf 87.837}	&	95.763 	&	{\bf 7.498} 	&	0.012 
	&	87.842 	&	{\bf 95.764} 	&	55.304 	&	0.435 	
	&	87.843 	&	95.765 	&	{\bf 19.779} 	&	0.435  \\
%($\bar{m}=5822$)
					& 		0.8	&	87.891 	&	95.676 	&	32.465 	&	0.188 	
					%&	87.905 	&	95.682 	&	{\bf 8.659} 	&	0.306 	
					&	87.882 	&	{\bf 95.634} 	&	75.384 	&	0.287 	
					&	{\bf 87.872} 	&	95.806 	&	{\bf 19.388} 	&	0.329  \\
%($n=85$)
					& 		0.5 	&	88.625 	&	95.562 	&	44.904 	&	0.859 	
					%&	{\bf 87.979}	&	95.502 	&	14.429 	&	0.788 	
					&	{\bf 88.101} 	&	{\bf 95.526} 	&	45.359 	&	0.675 	
					&	88.211 	&	96.592 	&	{\bf 5.453} 	&	0.871  \\ \hline
%					& \tred{wCw}	&	{\bf 87.920}	&	95.694 	&	{\bf 50.714} 	&	0.000 
%					%&	88.435 	&	93.727 	&	{\bf 24.099}	&	0.882 
%						&	(F)93.009 	&	101.243 	&	300.000 	&	0.141
%						 	&	---	&	---	&	---	&	--- \\\hline 

{\bf Student} 				& 		1	&	{\bf 1.127} 	&	{\bf 0.778} 	&	{\bf 10.586} 	&	0.625
 	%&	{\bf 1.126}	&	0.778 	&	32.335 	&	0.801
 	 	&	1.147 	&	0.785 	&	217.415 	&	0.032 	
 	 	&	1.147 	&	0.785 	&	81.766 	&	0.066 \\

					& 	0.8 	&	1.083 	&	{\bf 0.724} 	&	{\bf 2.348} 	&	0.996 	
					%&	{\bf 1.082} 	&	0.724 	&	34.236 	&	0.996 
						&	{\bf 1.082} 	&	{\bf 0.724} 	&	409.382 	&	0.004 	
						&	1.100 	&	0.731 	&	241.298 	&	0.004 \\

					& 	0.5	&	{\bf 1.082} 	&	{\bf 0.724} 	&	{\bf 3.618} 	&	0.996 	
					%&	1.082 	&	0.724 	&	48.922 	&	0.996 	
					&	1.125 	&	0.772 	&	152.826 	&	0.829 	&	2.848 	&	1.120 	&	9.520 	&	0.974 \\ \hline
%					& \tred{ wCw}	&	{\bf 1.132} 	&	0.771 	&	{\bf 1.451} 	&	0.368 
%						%&	(F)1.318 	&	0.509 	&	300.000 	&	0.563 	
%						&	(F)21.003 	&	18.324 	&	300.000 	& 	---	&	---	&	---	&	---	&---	\\\hline 
{\bf BodyFat} 				&		1	&	0.277 	&	{\bf 0.209} 	&	{\bf 0.068} 	&	0.071 	
%&	0.277 	&	0.209 	&	2.556 	&	0.071 
	&	{\bf 0.276} 	&	0.210 	&	10.253 	&	0.714 	&	0.279 	&	0.216 	&	0.820 	&	0.714 \\
%($\bar{m}=$)
%$(\lambda^0=10)$ 		
                   			& 		0.8	&	0.288 	&	{\bf 0.179} 	&	{\bf 0.203} 	&	0.000
                   			 	%&	0.778 	&	0.860 	&	3.176 	&	0.857 
                   			 		&	{\bf 0.280} 	&	0.184 	&	10.567 	&	0.571 	&	0.287 	&	0.182 	&	0.808 	&	0.429 \\
%($n=$)
					& 		0.5 	&	0.582 	&	0.267 	&	{\bf 0.395} 	&	0.714 
						%&	1.280 	&	0.981 	&	3.381 	&	0.929 	
						&	0.353 	&	0.229 	&	7.279 	&	0.286
						&	{\bf 0.316} 	&	{\bf 0.256} 	&	0.931 	&	0.286 \\ \hline
%					& wCw	&	{\bf 0.531} 	&	0.243 	&	{\bf 0.072} 	&	0.000 	
%					%&	{\bf 0.292} 	&	0.123 	&	5.158 	&	0.357 	
%					&	(F)27.387 	&	27.437 	&	300.000 	&	0.929 	&	---	&	---	&	---	&	--- \\\hline 

{\bf CpuSmall} 				&1 	&	132326	&	{\bf 130981} 	&	11.299 	&	0.083 	
%&	132326	&	130981	&	{\bf 5.092} 	&	0.083 	
&	{\bf 131834}	&	131123 	&	21.334 	&	0.917 	
&	132261	&	130983	&	{\bf 1.164} 	&	0.917 \\
%($\bar{m}=$)
					& 0.8 	&	132339 	&	{\bf 130982}	&	{\bf 0.741} 	&	0.250 
						%&	132339 	&	130982 	&	5.001 	&	0.250 	
						&	{\bf 131770} 	&	131187 	&	19.909 	&	0.917 	
						&	132205 	&	130991 	&	1.240 	&	0.750 \\
%($n=$)
					& 0.5	&	132093	&	{\bf 131058} 	&	{\bf 0.672} 	&	0.250 	
					%&	132093 	&	131058 	&	5.184 	&	0.250 	
					&	{\bf 131754}	&	131234	&	17.619 	&	0.917 
				  &	132127 	&	131059 	&	1.514 	&	0.750 \\ 
%					& wCw	&	{\bf 132780}	&	131130 	&	{\bf 6.222} 	&	0.000
%					 	%&	{\bf 131940}	&	128540 	&	{\bf 4.581} 	&	0.750 	
%					 	&	(F)153100 	&	151150 	&	300.000 	&	1.000 
%					 		&	---	&	---	&	---	&	--- \\ %\hline 
\bottomrule
\end{tabular}}}
\end{table}
\end{landscape}


==> backup/tablewatanabe2.tex <==

\begin{landscape}
  \begin{table}[h]
\centering
\caption{  
 Comparison of \texttt{bayesopt} and Algorithm	s~\ref{alg:smoothing} using the implicit function approach and \texttt{fmincon} as subroutines for solving subproblem\,\eqref{eqn:smoothprob} in Step~2 in terms of squared errors (validation error ${\rm Err}_{\rm val}$ and test error ${\rm Err}_{\rm te}$), CPU times (time(sec)), and sparsities (sparsity).
Here, ${\rm sparsity}:=\left|\{i\mid w_i=0\}\right|/n$ and hence 
a solution is sparser as ``{\rm sparsity}'' is closer to 1.
{\algone} stands for Algorithm~\ref{alg:smoothing} using the implicit function approach and
{\algtwo} does the one using \texttt{fmincon}.
The notation $\sharp \blambda$ stands for the number of hyperparameters in each problem. 
Moreover, the best values in ${\rm Err}_{\rm val}$, ${\rm Err}_{\rm te}$, and time(sec) are displayed in bold.
The hyphens ``--'' for {\bf Facebook} indicate that \texttt{fmincon}, which is used in {\algtwo}, terminates with an infeasible solution of the smoothed problem\,\eqref{eqn:smoothprob}.
The algorithms with ``600'' seconds stopped at the time-limit.
}
\label{tbl2:comparison_full}
	{
\scalebox{1}{%ワタナベが付け加えた
\begin{tabular}{lrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{2}{c}{Data}&
\multicolumn{4}{c}{{\algone}}&
\multicolumn{4}{c}{{\algtwo}}&
\multicolumn{4}{c}{\texttt{bayesopt} in MATLAB}\\
\cmidrule(lr){1-2}
\cmidrule(lr){3-6}
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
\multicolumn{1}{c}{name}&
\multicolumn{1}{c}{$\sharp\blambda$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm te}$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)}&
\multicolumn{1}{c}{sparsity}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm te}$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)} &
\multicolumn{1}{c}{sparsity}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm te}$}&
\multicolumn{1}{c}{$\mbox{Err}_{\rm val}$}&
\multicolumn{1}{c}{time (sec)}&
\multicolumn{1}{c}{sparsity}\\
\midrule
{\bf Facebook}				&	54 & 	{\bf 5.404} 	&	6.478 	&	{20.247}	&	0.038 	
					        &	--&	--&	-- &	-- 
&	7.629 	&	8.780 	&	600.000 	&	0.000 \\\hline
{\bf Insurance}					& 86 	&	{\bf 87.920}	&	95.694 	&	{50.714} 	&	0.000 
&	88.340 	&	{\bf 94.604} 	&	{\bf 4.473}	&	0.988
						& 98.000 	&	107.000 	&	600.000 	&	0.000\\\hline
{\bf Student}				& 273&	{\bf 1.132} 	&	{\bf 0.771} 	&	{\bf 1.451} 	&	0.368 
&	1.142 	&	0.786 	&	71.775 	&	0.670
&	21.002 	&	18.324 	&	600.000 &0.000\\\hline
{\bf BodyFat}					& 15 	&	{0.531} 	&	0.243 	&	{\bf 0.072} 	&	0.000 	
&	{\bf 0.286} 	&	{\bf 0.130} 	&	0.695 	&	0.933
&	46.675 	&	48.815 	&	455.230 	&	0.000\\\hline
{\bf CpuSmall}					& 13 	&	{132780}	&	131130 	&	{6.222} 	&	0.000
&	{\bf 131940}	&	{\bf 128540} 	&	{\bf 0.658} 	&	0.692
					 	&	156420 	&	151670 	&	600.000 	&	1.000 \\
\bottomrule
\end{tabular}}}
\end{table}
\end{landscape}


==> backup/theoreticalGuarantee.tex <==
\section{Theoretical Results}\label{sec:theory}
In this section, we will prove the global convergence of Algorithm\,\ref{alg:smoothing} by investigating an accumulation point of a sequence generated by that algorithm.
  For this purpose, in Section\,\ref{SB-KKT}, we first present new optimality conditions for the original bilevel problem\,\eqref{eqn:bilevel}, named {\it scaled bilevel KKT (SB-KKT)} conditions.
Moreover, in Section~\ref{sec:convtoSB}, we prove that any accumulation point of a sequence generated by Algorithm\,\ref{alg:smoothing} actually satisfies the SB-KKT conditions under some assumptions.
%we begin with deriving a certain one-level optimization problem from \eqref{eqn:bilevel}.
%For that problem, we prove that the SB-KKT conditions are nothing but necessarily optimality conditions. 

%% In this section, for the original bilevel problem\,\eqref{eqn:bilevel},
%% we present new optimality conditions, named {\it scaled bilevel KKT (SB-KKT)} conditions. 
%% To this end, 

Throughout the section, we often use the following notations for $\w\in \R^n$:
\begin{align*}
I(\w):=\{i\in \{1,2,\ldots,n\}\mid w_i=0\},\ |\bw|^{p}:=\left(|w_1|^p,|w_2|^p,\ldots,|w_n|^p\right)^{\top}.
\end{align*}
\subsection{SB-KKT Conditions}\label{SB-KKT}
Now, we define the SB-KKT conditions for problem\,\eqref{eqn:bilevel}:
\begin{definition}
We say that the scaled bilevel 
Karush-Kuhn-Tucker (SB-KKT) conditions hold at $(\w^{\ast},\blambda^{\ast})\in \R^n\times \R^r$ 
for problem\,\eqref{eqn:bilevel}
when there {exists a pair of vectors} $(\bzeta^{\ast},\bbeta^{\ast})\in \R^n\times\R^r$ such that
\begin{eqnarray}
  &\bW_{\ast}^2\nabla f(\w^{\ast})+\H(\w^{\ast},\blambda^{\ast})\bzeta^{\ast}=\0,\label{eqa:1214-1}\\
&\bW_{\ast}\nabla_{\w}G({\w}^{\ast},\bar{\blambda}^{\ast})+p\lambda_1^{\ast}|\bw^{\ast}|^p=\0,\label{eqa:1214-2}\\
& p\sum_{i\notin I(\w^{\ast})}{\rm sgn}(w_i^{\ast})|w_i^{\ast}|^{p-1}\zeta_i^{\ast}=\eta_1^{\ast},\label{eqa:1214-3}\\
&\zeta_i^{\ast}=0\ (i\in I(\w^{\ast})),\label{eqa:1214-6}\\
&\nabla R_i(\w^{\ast})^{\top}\bzeta^{\ast}=\eta_i^{\ast}\ \ (i=2,3,\ldots,r),\label{eqa:1224-4}\\ 
&\0\le \blambda^{\ast}, ~\0 \le \bbeta^{\ast}, ~(\blambda^{\ast})^\top \bbeta^{\ast}=0,\label{eqa:1214-5}
\end{eqnarray}
where 
$\bW_{\ast}:={\rm diag}(\bw^{\ast})$.
Here, we write 
$$
\H(\w,\blambda):=\bW^2\nabla^2_{\bw}G(\w,\bar{\blambda})+\lambda_1p(p-1)\diag(|\bw|^p)
$$ 
{with $\bW:={\rm diag}(\bw)$} {for $\w\in \R^n$ and $\blambda\in \R^r$.}
In particular, we call 
{a point $(\bw^{\ast},\blambda^{\ast})\in \R^n\times \R^r$}
satisfying the above conditions\,\eqref{eqa:1214-1}--\eqref{eqa:1214-5} an SB-KKT point for problem\,\eqref{eqn:bilevel}.
\end{definition}

In fact, $(\0,\blambda^{\ast})$ is a trivial SB-KKT point for any $\blambda^{\ast}$.
  This can be checked by setting $(\bzeta^{\ast},\bbeta^{\ast})=(\0,\0)$ in the conditions\,\eqref{eqa:1214-1}--\eqref{eqa:1214-5}.
  Experimentally, started from a point apart from such a trivial point, Algorithm~\ref{alg:smoothing} finds non-trivial SB-KKT points in many cases.   


{We next prove that the SB-KKT conditions are necessary optimality conditions 
for a certain one-level problem. For this purpose, we derive the {\it scaled first-order necessary condition}\,\citep{chen2010lower} for the lower-level problem in \eqref{eqn:bilevel}:
\begin{equation}
\min_{\bm w \in \R^n}G(\w,\bar{\blambda})+\lambda_1\|\w\|^p_p.\label{eq:low}
\end{equation}
{We say that 
the scaled first-order necessary condition of \eqref{eq:low} holds at $\w^{\ast}$ if}
\begin{equation}
  \bW_{\ast}\nabla_{\w}G(\w^{\ast},\bar{\blambda})+p\lambda_1|\bw^{\ast}|^p= \bm 0.\label{eq:scaled_first}
\end{equation}
%where $\bW_{\ast}={\rm diag}(\w^{\ast})$.
Indeed, a local optimum $\w^{\ast}$ of \eqref{eq:low} satisfies the above condition.
This fact can be verified easily by following the proof of Theorem~2.1 in \citep{chen2010lower}.
The above scaled condition was originally presented in
\citep{chen2010lower,chen2013optimality,bian2017optimality} for some optimization problems admitting non-Lipschitz functions.


As in deriving \eqref{eq:0615-2056},
we obtain the following one-level problem by replacing the lower problem in \eqref{eqn:bilevel} with
the scaled first-order necessary condition \eqref{eq:scaled_first}:
\begin{equation}
\displaystyle\min_{\w,\blambda}\ f(\w)\hspace{0.5em}\mbox{s.t.}\hspace{0.5em}\bW \nabla_{\w}G(\w,\bar{\blambda})+p\lambda_1|\bw|^p= \bm 0,\ \blambda\ge \0.
\label{eqn:surrogate}
\end{equation}
%where ${\bm W}={\diag}(\bm w)$.
As well as \eqref{eq:0615-2056}, the feasible region of \eqref{eqn:surrogate} includes not only 
the global optimal solution of the lower-level problem in the original problem \eqref{eqn:bilevel} but also its local solutions.
Notice that the above problem is still nonsmooth due to the existence of $|\bw|^p$. 

The following theorem states that the SB-KKT conditions are necessary optimality conditions for \eqref{eqn:surrogate}.}
Here, we just give an outline of the proof and defer its detail to Appendix~\ref{appendix:kkt}.\\
%\eqref{eqn:surrogate}.
\begin{theorem}\label{thm:optimality}
Let $(\w^{\ast},\blambda^{\ast})\in \R^n\times \R^r$ be a local optimum of %\eqref{eq:0615-2056}.
\eqref{eqn:surrogate}.
Then,
$(\w^{\ast},\blambda^{\ast})$ together with some vectors
$\bzeta^{\ast}\in \R^n$ and $\bbeta^{\ast}\in\R^r$ satisfies the 
SB-KKT conditions\,\eqref{eqa:1214-1}--\eqref{eqa:1214-5}
under an appropriate constraint qualification concerning the constraints 
$\frac{\partial{G(\w,\bar{\blambda})}}{\partial w_i}+p\,{\rm sgn}(w_i)\lambda_1|w_i|^{p-1}=0\ (i\notin I(\w^{\ast})),\ w_i=0\ (i\in I(\w^{\ast}))${, and $\blambda\ge \bm 0$}.
\end{theorem}
    {\noindent{\bf{Sketch of the proof}}: Notice that $(\w^{\ast},\blambda^{\ast})$ is a local optimum of the following problem:
\begin{align}\label{eqn:surrogate2}
\begin{array}{rcc}
\displaystyle\min_{\w,\blambda}&  & f(\w)  \\
\mbox{s.t.} &     &\displaystyle \frac{\partial{G(\w,\bar{\blambda})}}{\partial w_i}+p\,{\rm sgn}(w_i)\lambda_1|w_i|^{p-1}=0\ (i\notin I(\w^{\ast}))\\
            &      &w_i=0\ (i\in I(\w^{\ast}))\\  
           &       &\blambda\ge \0.
\end{array}
\end{align}
This is because  
$(\w^{\ast},\blambda^{\ast})$ is also feasible to \eqref{eqn:surrogate2} and the feasible region of 
\eqref{eqn:surrogate} is larger than that of \eqref{eqn:surrogate2}.
Hence, the KKT conditions hold at $(\w^{\ast},\blambda^{\ast})$ for \eqref{eqn:surrogate2} in the presence of a constraint qualification.
Finally, these KKT conditions can be equivalently transformed into the desired SB-KKT conditions.}
\hfill$\blacksquare$


In the next section, we will study convergence analysis of Algorithm~\ref{alg:smoothing} to an SB-KKT point.
Before proceeding to the convergence analysis, let us see the relationship between the two one-level problems
\,\eqref{eq:0615-2056} and \eqref{eqn:surrogate}. 
The following lemma concerns the feasible regions of \eqref{eq:0615-2056} and \eqref{eqn:surrogate}.
\begin{LEMM}\label{lem:0708-2352}
For $\w\in \R^n$ and $\blambda\in \R^r_+$, 
if 
$\bm 0\in \partial_{\w}(G(\w,\bar{\blambda})+\lambda_1R_1(\w))$,
then  $\bW \nabla_{\w}G(\w,\bar{\blambda})+p\lambda_1|\bw|^p= \bm 0$. 
In particular, when $p<1$, the converse is also true.
\end{LEMM}
\begin{proof}
See Appendix~\ref{appendix:lemma}. 
\end{proof}
In view of the above lemma, we find that 
the feasible region of \eqref{eqn:surrogate} is larger than that of \eqref{eq:0615-2056} in general. 
However, for the case of $p<1$, we also see that these two regions are identical.  These relationships are summarized as in the following diagram.
\begin{equation*}
\mbox{Feasible region of \eqref{eqn:bilevel}} \subseteq \mbox{Feasible region of }\eqref{eq:0615-2056} 
\left\{\begin{array}{c}
\subseteq_{p=1}\\
=_{p<1}
\end{array}\right\}
 \mbox{Feasible region of }\eqref{eqn:surrogate}.
\end{equation*}
From this observation and Theorem\,\ref{thm:optimality}, we can derive the following theorem immediately: 
\begin{theorem}
Let $p<1$ and $(\w^{\ast},\blambda^{\ast})\in \R^n\times \R^r$ be a local optimum of \eqref{eq:0615-2056}.
Then,
$(\w^{\ast},\blambda^{\ast})$ together with some vectors
$\bzeta^{\ast}\in \R^n$ and $\bbeta^{\ast}\in\R^r$ satisfies the 
SB-KKT conditions\,\eqref{eqa:1214-1}--\eqref{eqa:1214-5}
under an appropriate constraint qualification concerning the constraints 
$\frac{\partial{G(\w,\bar{\blambda})}}{\partial w_i}+p\,{\rm sgn}(w_i)\lambda_1|w_i|^{p-1}=0\ (i\notin I(\w^{\ast})),\ w_i=0\ (i\in I(\w^{\ast}))${, and $\blambda\ge \bm 0$}.
\end{theorem}
 
\subsection{Convergence of Algorithm~\ref{alg:smoothing} to an SB-KKT Point}\label{sec:convtoSB}
Hereafter, 
for convenience of explanation,
we suppose that 
an $\hat{\varepsilon}_{k-1}$-approximate KKT point 
$(\w^k, \blambda^k,\bzeta^{k},\bbeta^{k})$
is a solution satisfying conditions\,\eqref{eq:1215-1}-\eqref{eq:1215-3}
with 
$$
(\bm\varepsilon_1,\varepsilon_2,{\bm \varepsilon}_3,{\bm\varepsilon}_4,\varepsilon_5)
=(\bm\varepsilon^{k-1}_1,\varepsilon_2^{k-1},{\bm \varepsilon}_3^{k-1},{\bm\varepsilon}_4^{k-1},\varepsilon_5^{k-1}),
$$
where $\{(\bm\varepsilon^{k}_1,\varepsilon_2^{k},{\bm \varepsilon}_3^{k},{\bm\varepsilon}_4^{k},\varepsilon_5^{k})\}$ is a sequence that converges to zero as $k\to \infty$.

Moreover, we suppose that the algorithm is well-defined in the sense 
that {an $\hat{\varepsilon}_k$-approximate} KKT point of \eqref{eqn:smoothprob} is found in Step~2 at every iteration, and
it generates {an} infinite number of iteration points.
In addition, we make the following assumptions:\vspace{1em}

\noindent{\bf Assumption~A:}\ Let {$\{(\w^k, \blambda^k,\bzeta^k,\bbeta^k)\}\subseteq \R^{n}\times \R^r
\times \R^{n}\times \R^r$
be a} sequence produced by the proposed algorithm. 
Then, the following properties hold:
\begin{enumerate}
\item[{\bf A1}:] ${\displaystyle \liminf_{k\to\infty}\lambda^k_1>0}$.
\item[{\bf A2}:] 
The sequence $\{(\w^k, \blambda^k,\bzeta^k,\bbeta^k)\}$ is bounded.
\item[{\bf A3}:] 
Let $p=1$ and $(\w^{\ast}, \blambda^{\ast})$
be an arbitrary accumulation point of the sequence $\{(\w^k, \blambda^k)\}$.
It then holds that $\lambda^{\ast}_1\neq \left|\frac{\partial G(\w^{\ast},\bar{\blambda}^{\ast})}{\partial w_i}\right|$ for any $i\in I(\w^{\ast})$.
\end{enumerate}
Assumption~A1 means that the $\ell_p$-regularization term, i.e., the function $R_1$ works effectively.
We will discuss Assumption~A2 at the end of this section.
  Specifically, we will prove that
under certain conditions, the Lagrange multiplier part $\{\bzeta^k,\bbeta^k)\}$ is actually bounded. 
Assumption~A3 is a technical assumption for the case of $p=1$.
It indicates that, for all $i\in I(\w^{\ast})$, zero is not situated on the boundary of the subdifferential of $G(\w,\blambda)+\lambda\|\w\|_1$ w.r.t. $w_i$.
Interestingly, for the case of $p<1$, we can establish the convergence of Algorithm~\ref{alg:smoothing} in the absence of A3. 

{Under the presence of these assumptions, our goal is to prove the following convergence theorem, which motivates us to make a stopping criterion of the algorithm based on the SB-KKT conditions in the numerical experiments we will conduct later.
\begin{theorem}\label{last_thm}
Suppose that Assumptions~A1--A3 hold.
Then, any accumulation point of $\{(\w^k,\blambda^k,{\bzeta^k},\bbeta^k)\}$
generated by Algorithm~\ref{alg:smoothing} satisfies the %bilevel scaled
SB-KKT conditions\,\eqref{eqa:1214-1}--\eqref{eqa:1214-5} for problem \eqref{eqn:bilevel}.
\end{theorem}
We will prove this theorem by showing that passing the approximate KKT conditions~\eqref{eq:1215-1}-\eqref{eq:1215-3} to the limit yields the SB-KKT conditions.
For this purpose, in particular, we have to examine how $\nabla\bphi_{\mu_k}(\w^k)$ and
$\nabla^2\bphi_{\mu_k}(\w^k)$ behave in the limit.
{We remark that each component of $\nabla\bphi_{\mu}(\w)$ and each diagonal one of $\nabla^2\bphi_{\mu}(\w)$ are expressed as 
\begin{align}
&(\nabla\bphi_{\mu}(\w))_i=pw_i(w_i^2+\mu^2)^{\frac{p}{2}-1},\label{al:1214-1}\\
&(\nabla^2\bphi_{\mu}(\w))_{ii}=p(w_i^2+\mu^2)^{\frac{p}{2}-1}+p(p-2)w_i^2(w_i^2+\mu^2)^{\frac{p}{2}-2}\label{al:1214-2} 
\end{align}
for $i=1,2,\ldots,n$, $\mu>0$, and $\w\in \R^n$.
Note that all the off-diagonal components of $\nabla^2\bphi_{\mu}(\w)$ are zeros.
We present the following proposition, whose proof is given in Appendix~\ref{appendix:Lemma2}.
\begin{proposition}\label{lem:1217-1}
Let $\w^{\ast}$ be the point defined in {\bf A3}.
Then, we have
\begin{align}
&\lim_{k\to\infty}\bW_k\nabla\bphi_{\mu_{k-1}}(\w^k)=p|\w^{\ast}|^p,\label{al:1214-1921}\\
&\lim_{k\to\infty}\bW^2_k\nabla^2\bphi_{\mu_{k-1}}(\w^k)=p(p-1)\diag(|\w^{\ast}|^p),\label{al:1214-1922}
\end{align}
where 
%\begin{align*}
${\bm W}_k:={\diag}(\bm w_k)$
for each $k$.
\end{proposition}}
Next, we prove that, for $i\in I(\w^{\ast})$, the $i$-th diagonal component of $(\nabla^2\bphi_{\mu_{k-1}}(\w^k))_{ii}$ diverges.
The key of its proof is the approach speed of $w_i\ (i\in I(\w^{\ast}))$ towards zeros compared with that of the smoothing parameter $\mu_{k-1}$.
Actually, according to the next lemma, $\mu_{k-1}$ gradually approaches $0$ with the speed not faster than $\max_{i\in I(\w^{\ast})}|w_i^k|^{\frac{1}{2-p}}$.
The proof will be given in Appendix~\ref{appendix:speed}.
Remarkably, when $p<1$, it holds true in the absence of Assumption\,{\bf A3}.
}
\begin{LEMM}\label{prop:0312}
Suppose that Assumptions~A1--A3 hold.
Let 
$(\w^{\ast},\blambda^{\ast})$ be an arbitrary accumulation point of 
$\{(\w^k,\blambda^k)\}$ and $\{(\w^k,\blambda^k)\}_{k\in K}(\subseteq \{(\w^k,\blambda^k)\})$ be an arbitrary subsequence converging to $(\w^{\ast},\blambda^{\ast})$.
Then, there exists some $\gamma > 0$ such that
\begin{equation}
\mu_{k-1}^2\ge \gamma |w_i^k|^{\frac{2}{2-p}} \ \ (i\in I(\w^{\ast}))\label{eq:A3}
\end{equation}
for all $k\in K$ sufficiently large.
\end{LEMM}
From the above lemma, we can derive the following proposition.
\begin{proposition}\label{lem:0312}
Suppose that Assumptions~A1--A3 hold. 
Let 
$\w^{\ast}$ be an arbitrary accumulation point of 
the sequence 
$\{\w^k\}$ and $\{\w^k\}_{k\in K}(\subseteq \{\w^k\})$ be an arbitrary subsequence converging to $\w^{\ast}$.
Then, for any $i\in I(\w^{\ast})$, 
\begin{equation}
\lim_{k\in K\to\infty}\left|(\nabla^2\bphi_{\mu_{k-1}}(\w^k))_{ii}\right|=\infty.\label{eq:0312:1012}
\end{equation} 
\end{proposition}
\begin{proof}
Choose $i\in I(\w^{\ast})$ arbitrarily.
Note that 
\begin{equation}
\lim_{k\in K\to \infty}|w^k_i|=w^{\ast}_i=0.\label{eq:0312-1540}
\end{equation}
By Lemma\,\ref{prop:0312}, 
there is some $\gamma>0$ such that 
\begin{equation}
\mu_{k-1}^2\ge \gamma|w^k_i|^{\frac{2}{2-p}}\label{eq:0312-1526}
\end{equation}
for all $k\in K$ sufficiently large. 
In view of this fact, we have, for all $k\in K$ large enough,
\begin{align}
\mu_{k-1}^2+(p-1)(w^k_i)^2&\ge  \gamma|w^k_i|^{\frac{2}{2-p}}+(p-1)|w^k_i|^2\notag \\ %\label{eq:0312-1438}
                        &= |w^k_i|^{\frac{2}{2-p}}(\gamma + (p-1)|w^k_i|^{2-\frac{2}{2-p}})\notag \\
                        &\ge 0, \label{al:0312-1504}
\end{align}
where the second inequality can be verified by noting that $\gamma + (p-1)|w^k_i|^{2-\frac{2}{2-p}}>0$ holds for all $k\in K$ sufficiently large because $\gamma>0$ and $(p-1)\lim_{k\in K\to \infty}|w^k_i|^{2-\frac{2}{2-p}}=
(p-1)|w_i^{\ast}|^{2-\frac{2}{2-p}}=0$. 
Furthermore, notice that
\begin{equation}
|w^k_i|^{\frac{2}{2-p}}\ge |w^k_i|^2\label{eq:0402-2}
\end{equation}
holds for all $k\in K$ sufficiently large because $1<\frac{2}{2-p}\le 2$ and 
$|w^k_i|<1$ for all $k\in K$ large enough by \eqref{eq:0312-1540}.
Relation\,\eqref{eq:0312-1526} then implies
\begin{equation}
\mu_{k-1}^2\ge \gamma|w^k_i|^{2}.\label{eq:0313-2}
\end{equation}
From expression\,\eqref{al:1214-2}, it follows that %\COMM{TO}{When changing $\mu_{k-1}^2$ to $\mu_{k-1}$, handle the part below with a great care to avoid any errors.} 
\begin{align}
\left|(\nabla^2\bphi_{\mu_{k-1}}(\w^k))_{ii}\right|
&=p\left|((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-2}\left((w^k_i)^2+\mu_{k-1}^2+(p-2)(w^k_i)^2\right)\right|
\notag\\
&=p \left|((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-2}(\mu_{k-1}^2+(p-1)(w^k_i)^2)\right|\notag\\
                                      &= p ((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-2}\left(\mu_{k-1}^2+(p-1)(w^k_i)^2\right)\notag \\
                                      &\ge  p \left(1+\frac{1}{\gamma}\right)^{\frac{p}{2}-2}\mu_{k-1}^{{p}-4}\left(\mu_{k-1}^2+(p-1)(w^k_i)^2\right)\notag\\
                                      &=  p \left(1+\frac{1}{\gamma}\right)^{\frac{p}{2}-2}\mu_{k-1}^{p-2}\left(1+(p-1)\frac{(w^k_i)^2}{\mu_{k-1}^2}\right),\label{al:0312-1444}
\end{align}
where the third equality follows from \eqref{al:0312-1504} and the first inequality comes from \eqref{eq:0313-2} and $\frac{p}{2}-2<0$.
Moreover, by \eqref{eq:0312-1526}, we see ${\mu_{k-1}^{2(2-p)}}/{\gamma^{2-p}}\ge (w^k_i)^2$
and thus have
\begin{equation}
\frac{\mu_{k-1}^{2-2p}}{\gamma^{2-p}}\ge \frac{(w^k_i)^2}{\mu_{k-1}^2}.\notag%\label{al:0312-1525}. 
\end{equation}
%where the first inequality follows from \eqref{eq:0312-1526}.
By this inequality, it holds that 
\begin{equation}
\lim_{k\in K\to \infty}\left|\frac{(w^k_i)^2}{\mu_{k-1}^2}\right|\begin{cases}=0\hspace{1em}&(p<1)\\
\le \frac{1}{\gamma}\hspace{1em}&(p=1).
\end{cases}
\notag
\end{equation}
Thus, we obtain  
\begin{equation}
\lim_{k\in K\to \infty}(p-1)\left|\frac{(w^k_i)^2}{\mu_{k-1}^2}\right|=0,\notag
\end{equation}
which together with \eqref{al:0312-1444} {and $\lim_{k\to \infty}\mu_{k-1}^{p-2}=\infty$} implies
\begin{equation}
\lim_{k\in K\to \infty}\left|(\nabla^2\bphi_{\mu_{k-1}}(\w^k))_{ii}\right|=\infty.\notag
\end{equation}
Since $i\in I(\w^{\ast})$ was arbitrarily chosen, the proof is complete.
\end{proof}

Now, we are ready to prove Theorem~\ref{last_thm} using Propositions~\ref{lem:1217-1} and \ref{lem:0312}.
\subsection*{Proof of Theorem~\ref{last_thm}}
Consider the $\hat{\varepsilon}_{k-1}$-approximate KKT conditions \eqref{eq:1215-1}, \eqref{eqn:1217-2}, and \eqref{eq:1215-2} with $(\w,\blambda,{\bzeta},\bbeta)=(\w^k,\blambda^k,{\bzeta^k},\bbeta^k)$ and
$({\bm \varepsilon}_1,
{\bm \varepsilon}_3,
{\varepsilon}_5)
=({\bm \varepsilon}^{k-1}_1,
{\bm \varepsilon}_3^{k-1},
{\varepsilon}_5^{k-1})$.
Let $(\w^{\ast},\blambda^{\ast},\bzeta^{\ast},\bbeta^{\ast})$ be an arbitrary accumulation point of $\{(\w^k,\blambda^k,\bzeta^k,\bbeta^k)\}$.
By taking a subsequence if necessary,
without loss of generality, we can suppose that
\begin{equation}
\lim_{k\to \infty}
(\w^k,\blambda^k,\bzeta^k,\bbeta^k)=(\w^{\ast},\blambda^{\ast},\bzeta^{\ast},\bbeta^{\ast}).\label{eq:conv}
\end{equation}
To show the desired result, it suffices to prove that $(\w^{\ast},\blambda^{\ast},\bzeta^{\ast},\bbeta^{\ast})$ satisfies \eqref{eqa:1214-1}--\eqref{eqa:1214-5}.
Now, we give the proof by three blocks as follows:\vspace{0.5em}\\
\noindent{\it Proof of conditions~\eqref{eqa:1214-1}, \eqref{eqa:1214-2}, \eqref{eqa:1224-4} and \eqref{eqa:1214-5}}:
As for \eqref{eqa:1214-1} and \eqref{eqa:1214-2}, multiplying
\eqref{eq:1215-1} and \eqref{eq:1215-2} {with $(\w,\blambda,{\bzeta},\bbeta)=(\w^k,\blambda^k,{\bzeta^k},\bbeta^k)$}
by $\bW_k^2$ and $\bW_k$ on the left, respectively, we obtain
\begin{align*}
&\bW_k^2\nabla f(\w^k) + \bW_k^2\left(\nabla_{\w\w}^2 G(\w^k,\bar{\blambda}^k)+\lambda_1^k \nabla^2\bphi_{\mu_{k-1}}(\w^k)\right){\bm\zeta^k}=\bW_k^2{\bm \varepsilon}^{k-1}_1,\\
&\bW_k \nabla_{\w} G(\w^k,\bar{\blambda}^k)+\lambda_1^k\bW_k \nabla\bphi_{\mu_{k-1}}(\w^k)={
\bW_k{\bm \varepsilon}^{k-1}_4}.
\end{align*}
Note that 
the functions $\nabla f$, $\nabla_{\w\w}^2 G$, and $\nabla_{\w} G$ are continuous and let $k\to \infty$ in the above equations. 
Then, using \eqref{al:1214-1921} and \eqref{al:1214-1922} in Proposition\,\ref{lem:1217-1} together with 
$\mu_{k-1}\to 0,\ 
{({\bm \varepsilon}^{k-1}_1,{\bm \varepsilon}^{k-1}_4)\to (\0,\0)
}$ as $k\to \infty$, 
we get \eqref{eqa:1214-1} and \eqref{eqa:1214-2}, that is to say,
\begin{align*}
  &\bW_{\ast}^2\nabla f(\w^{\ast}) +\H(\w^{\ast},\blambda^{\ast})\bzeta^{\ast}=\0, \\
&\bW_{\ast}\nabla_{\w}G(\w^{\ast},\bar{\blambda}^{\ast})+p\lambda_1^{\ast}|\bw^{\ast}|^p=\0.
\end{align*}
Conditions\,\eqref{eqa:1224-4} and \eqref{eqa:1214-5} are obtained by driving $k$ to $\infty$ in \eqref{eqn:1217-2} and \eqref{eq:1215-3} {with $(\w,\blambda,{\bzeta},\bbeta)=(\w^k,\blambda^k,{\bzeta^k},\bbeta^k)$}.\vspace{0.5em}

\noindent{\it Proof of condition~\eqref{eqa:1214-6}}:
%% As for the remaining conditions~\eqref{eqa:1214-3} and \eqref{eqa:1214-6},
%% we leave the complet proof to Appendix~\ref{appendix:lastthm} and omit it here since they can be shown in a manner similar to the argument for showing \eqref{eq:0605-4} and \eqref{eq:0607-2} in the proof of Proposition\,\ref{prop:0607}.
%The next proposition concerns the validity of the condition \eqref{eqa:1214-3} at an accumulation point of the sequence generated by the algorithm.
%The proof is partially similar to the argument for showing \eqref{eq:0605-4} and \eqref{eq:0607-2} in the proof of Proposition\,\ref{prop:0607}. 
%But, for the sake of completeness of the paper, we give its proof without omitting it.
%% \begin{enumerate}
%% \item\label{Lem:item2} $\zeta_i^{\ast}=0$ for all $i\in I(\w^{\ast})$, and 
%% \item\label{Lem:item1}
%% $(\w^{\ast},\blambda^{\ast},\bzeta^{\ast},\bbeta^{\ast})$ 
%% satisfies the condition \eqref{eqa:1214-3}.
%% \end{enumerate}
%% The boundedness of the sequence $\{(\w^k,\blambda^k,\bzeta^k,\bbeta^k)\}$ follows from Proposition~\ref{prop:0607} and Assumption~A2.
%% Hence, the first claim is verified.
%By taking a subsequence if necessary, without loss of generality, we can suppose that
%\begin{equation}
%\lim_{k\to \infty}
%(\w^k,\blambda^k,\bzeta^k,\bbeta^k)=(\w^{\ast},\blambda^{\ast},\bzeta^{\ast},\bbeta^{\ast}).\label{eq:conv}
%\end{equation}
%We show item~\ref{Lem:item2}.
Choose $i\in I(\w^{\ast})$ arbitrarily.
Note that the continuity of the functions $\nabla^2_{\w\w}G$ and $\nabla f$.
Then, from \eqref{eq:conv} and condition\,\eqref{eq:1215-1} with $(\w,\blambda,\bzeta)=(\w^k,\blambda^k,\bzeta^k)$, $\{\lambda^k_1 \left(\nabla^2\bphi_{\mu_{k-1}}(\w^k)\right)_{ii}{\zeta^k_i}\}$ is bounded.
On the other hand, recall that  $\{(\nabla^2\bphi_{\mu_{k-1}}(\w^k))_{ii}\}$ is unbounded from Proposition\,\ref{lem:0312}
and $\lim_{k\to\infty}\lambda^k_1=\lambda^{\ast}_1>0$ from Assumption~A1. 
Thus, we get $\lim_{k\to\infty}\zeta^k_i=0$. 
Since the index $i$ was chosen from $I(\w^{\ast})$ arbitrarily, we conclude condition~\eqref{eqa:1214-6}.\vspace{0.5em}

\noindent{\it Proof of condition~\eqref{eqa:1214-3}:} We begin with proving 
\begin{equation}
\lim_{k\to\infty}\sum_{i\in I(\bw^{\ast})}w^k_i((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-1}\zeta^k_i=0. \label{eq:1217-2340}
\end{equation}
Choose $i\in I(\w^{\ast})$ arbitrarily again.
Note that by Lemma\,\ref{prop:0312}, there exists some $\gamma>0$ such that 
\begin{equation}
\mu_{k-1}^2\ge \gamma|w^k_i|^{\frac{2}{2-p}}\label{eq:0312-1818}
\end{equation}
for all $k$ sufficiently large. In what follows, we consider sufficiently large $k$ so that the 
inequality \eqref{eq:0312-1818} holds.
Then, by $0< p\le 1$, we get 
\begin{equation}
\frac{\mu_{k-1}^{2-p}}{\gamma^{\frac{2-p}{2}}}\ge |w^k_i|.\label{eq:0312-1818-2}
\end{equation}
We then have  
\begin{align}
\left|w^k_i((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-1}\zeta^k_i\right|&\le \left|w^k_i\mu_{k-1}^{2(\frac{p}{2}-1)}\zeta^k_i\right|\notag \\
&\le \frac{\mu_{k-1}^{2-p}}{\gamma^{\frac{2-p}{2}}}\mu_{k-1}^{2(\frac{p}{2}-1)}\left|\zeta^k_i\right|\notag\\
&=\gamma^{\frac{p}{2}-1}\left|\zeta^k_i\right|.\label{al:1216:2340}
\end{align}
Relation\,\eqref{al:1216:2340} and condition~\eqref{eqa:1214-6}, which was proved above, imply
\begin{equation*}
\lim_{k\to\infty}\left|w^k_i((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-1}\zeta^k_i\right|=0\label{eq:0312-1828}
\end{equation*}
and hence summing up this equation over $I(\w^{\ast})$ gives the desired expression\,\eqref{eq:1217-2340}}.

  Next, by using \eqref{eq:conv}, $\mu_{k-1}\to 0\ (k\to\infty)$, $w_i^{\ast}\neq 0\ (i\notin I(\w^{\ast}))$, and
$w^{\ast}_i={\rm sgn}(w^{\ast}_i)|w^{\ast}_i|$, we obtain 
\begin{align}
&\lim_{k\to\infty}\sum_{i\notin I(\bw^{\ast})}w^k_i((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-1}\zeta^k_i\notag \\
&=\sum_{i\notin I(\bw^{\ast})}{\rm sgn}(w^{\ast}_i)|w^{\ast}_i|^{p-1}\zeta^{\ast}_i.\label{eq:1216-2357}
\end{align}
Combining \eqref{eq:1217-2340} and \eqref{eq:1216-2357} with \eqref{al:1214-1} yields 
\begin{align*}
&\lim_{k\to\infty}\nabla\bphi_{\mu_{k-1}}(\w^k)^{\top}\bzeta^k\\
&=
\lim_{k\to\infty}p\sum_{i=1}^nw^k_i((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-1}\zeta^k_i\\
&=p\lim_{k\to\infty}\left(\sum_{i\in I(\w^{\ast})}w^k_i((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-1}\zeta^k_i
+\sum_{i\notin I(\w^{\ast})}w^k_i((w^k_i)^2+\mu_{k-1}^2)^{\frac{p}{2}-1}\zeta^k_i
\right)
\\
&=p \sum_{i\notin I(\bw^{\ast})}{\rm sgn}(w^{\ast}_i)|w^{\ast}_i|^{p-1}\zeta^{\ast}_i,
\end{align*}
which together with 
driving $k$ to $\infty$ in condition\,\eqref{eqn:1217-1} with $(\w,\blambda,\bzeta,\bbeta)=(\w^k,\blambda^k,\bzeta^k,\bbeta^k)$
implies
\begin{equation*}
p \sum_{i\notin I(\bw^{\ast})}{\rm sgn}(w^{\ast}_i)|w^{\ast}_i|^{p-1}\zeta^{\ast}_i=\eta_1^{\ast},
\end{equation*}
where we use $\eta^{\ast}_1=\lim_{k\to \infty}\eta^k_1$.
This is nothing but condition\,\eqref{eqa:1214-3}.

Consequently, the proof of Theorem~\ref{last_thm} is complete.\\
\hfill$\blacksquare$

{\subsection*{Boundedness of the Lagrange-multiplier Sequence}
  In Assumption~{\bf A2},
  we suppose that the Lagrange multiplier sequence $\{(\bzeta^k,\bbeta^k)\}$ is bounded.
One may ask when this condition holds. 
In many optimization algorithms, boundedness properties of relevant Lagrange multiplier sequences are shown to be true under suitable constraint qualifications.
In fact, we can verify the boundedness of $\{(\bzeta^k,\bbeta^k)\}$ under the presence of linearly constraint-like qualifications as follows:
\begin{description}
\item[{\bf A4}:] 
Let $(\w^{\ast},\blambda^{\ast})\in \R^n\times \R^r$ be an arbitrary accumulation point of the sequence $\{(\w^k,\blambda^k)\}$.
{Let 
$$I(\blambda^{\ast}):=\{i\in\{1,2,\ldots,r\}\mid \lambda_i^{\ast}=0\}.$$}
Then, the linearly independent constraint qualification (LICQ) holds at $(\w,\blambda)=(\w^{\ast},\blambda^{\ast})$ for the constraints 
${\Phi_{i}(\w,\blambda):=}\frac{\partial{G(\w,\bar{\blambda})}}{\partial w_i}+p\,{\rm sgn}(w_i)\lambda_1|w_i|^{p-1}=0\ (i\notin I(\w^{\ast})),\ w_i=0\ (i\in I(\w^{\ast}))$, and $\blambda\ge \bm 0$,
{that is to say, the gradient vectors for the active constraints 
$$\left\{
\left\{\nabla \Phi_{i}(\w^{\ast},\blambda^{\ast})\right\}_{i\notin I(\w^{\ast})},
\left\{\nabla_{(\w,\blambda)} w_i|_{\w = \w^{\ast}}\right\}_{i\in I(\w^{\ast})},
\left\{\nabla_{(\w,\blambda)} \lambda_i|_{\blambda=\blambda^{\ast}}\right\}_{i\in I(\blambda^{\ast})}
\right\}\subseteq \R^{n+r}
$$
are linearly independent.
}
\end{description}

\begin{proposition}\label{prop:0607}
  Suppose that Assumptions~A1, A3, and A4 hold.
  Additionally, suppose that the sequence $\{(\w^k,\blambda^k)\}$ is bounded.
Let $\{(\bzeta^k,\bbeta^k)\}\subseteq \R^{n}\times \R^r$ be a sequence of the accompanying Lagrange multiplier vectors which satisfy the KKT conditions\,\eqref{eq:1215-1}--\eqref{eq:1215-3}.
Then, $\{(\bzeta^k,\bbeta^k)\}$ is bounded.
\end{proposition}
\begin{proof}
  We derive contradiction by supposing that $\{(\bzeta^k,\bbeta^k)\}$ is unbounded.
For details, see Appendix~\ref{appendix:boundedness}.
\end{proof}}

